Completing Visual Objects via Bridging Generation and Segmentation

This paper presents a novel approach to object completion, with the primary goal of reconstructing a complete object from its partially visible components. Our method, named MaskComp, delineates the completion process through iterative stages of generation and segmentation. In each iteration, the object mask is provided as an additional condition to boost image generation, and, in return, the generated images can lead to a more accurate mask by fusing the segmentation of images. We demonstrate that the combination of one generation and one segmentation stage effectively functions as a mask denoiser. Through alternation between the generation and segmentation stages, the partial object mask is progressively refined, providing precise shape guidance and yielding superior object completion results. Our experiments demonstrate the superiority of MaskComp over existing approaches, e.g., ControlNet and Stable Diffusion, establishing it as an effective solution for object completion.

==> icml2024/src/0-abs.tex <==
This paper presents a novel approach to object completion, with the primary goal of reconstructing a complete object from its partially visible components. Our method, named \textbf{\textsl{MaskComp}}, delineates the completion process through iterative stages of generation and segmentation. 
In each iteration, the object mask is provided as an additional condition to boost image generation, and, in return, the generated images can lead to a more accurate mask by fusing the segmentation of images.
We demonstrate that the combination of one generation and one segmentation stage effectively functions as a mask denoiser. Through alternation between the generation and segmentation stages, the partial object mask is progressively refined, providing precise shape guidance and yielding superior object completion results. Our experiments demonstrate the superiority of MaskComp over existing approaches, \eg, ControlNet and Stable Diffusion, establishing it as an effective solution for object completion.

% each iter, mask as input, image boost next generation, (generation based on mask, why iteration, generate multiple, fuse for better segm for next, in this way both segm and gen improved)
% In each iteration, the object mask is provided as an additional condition to boost the image generation and, in return, the generated images can lead to a more accurate mask by fusing the segmentation of them.
% In this process, the partial object serves as contextual information for the object generation, while segmentation augments the process by offering crucial shape guidance. 
% gen multi sample can enhance mask (mutual benefit, two insight)
% We demonstrate that the combination of one generation and one segmentation stage effectively functions as a mask denoiser. Through alternation between the generation and segmentation stages, the partial object mask progressively refines, providing precise shape guidance and yielding superior object completion results. Our experiments demonstrate the superiority of MaskComp over existing approaches, \eg, ControlNet and Stable Diffusion, establishing it as an effective solution for object completion.

==> icml2024/src/1-intro.tex <==
\section{Introduction}

\begin{figure*}[t]
    \centering    
    \includegraphics[width=\linewidth]{figs/teaser.pdf}
    \vspace{-0.7cm}
    \caption{\textbf{Illustration of iterative mask denoising (IMD).} Starting from an initial partial object and its corresponding mask, IMD utilizes alternating generation and segmentation stages to progressively refine the partial mask until it converges to the complete mask. With the complete mask as the condition, the final complete object can be seamlessly generated.
    % cat one row, add text candidates
    % add the added part in the partial mask (mask denoising)
    % mask from partial to complete, image from noisy to clear
    % put on the second page
    % first page put a qualitative result
    % \ca{use image input for mask denoising, use mask for image denoising, why beneficial? mask for shape prior, image for distribution}
    }
    \label{fig:teaser}
\end{figure*}

% 1. how gen benefit segm
% 2. how segm benefit gen

% intro story:
% 1. mask avg -> better
% 2. how to avg img?
% 3. Progressive Masked Revision

% object completion: 
% 1. mask better -> completion better (exp: mask -> diff better)
% 2. Iteratively (gen img + avg mask) -> mask better (exp: diff -> improve mask, mask off-the-shelf segm is ok -> good generalization)
% 3. after first 1,2, then EM
% 4. explain mask avg and not diff img
% 5. explain mask better lead to better gen
% 6. teaser present （1，2），multiple mask avg -> mask better + gen image variation smaller
% 7. first page (G-step, S-step), second page (details of G- and S-step)
% 8. don't mention amodal segmentation
% 9. controller, cannot complete occluded obj (gap)

% Creative image editing has attracted extensive attention in recent years. Recent advances in image generation enable compelling results for various image editing tasks, such as image inpainting \citep{}, composition \citep{}, colorization \citep{} and aesthetic enhancement \citep{}. A more challenging scenario, on the other hand, is object completion, which intends to complete occluded objects in an image while preserving the object realism. Compared to image inpainting which incorporates complete objects into images, object completion requires a more fine-grained understanding of the objects to ensure completeness.

% In recent years, creative image editing has garnered significant attention and witnessed notable advancements. Current research has predominantly focused on manipulating the visible pixels within images, resulting in remarkable achievements such as image inpainting \citep{Xie_2023_CVPR}, composition \citep{yang2023paint}, and colorization \citep{Chang_2023_CVPR}. However, there exists a relative neglect in the exploration of modifying images in the depth direction, considering them as layered stacks of objects and background. Due to the occlusion, the objects in the image are always incomplete, making it necessary to complete the objects before the depth-level editing. Diverging from other conditional generation tasks, such as image inpainting, which solely generates and integrates complete objects into images, object completion demands a seamless alignment between the generated content and the provided partial object. This necessity imposes additional challenges in the pursuit of achieving realistic and comprehensive object shapes.

% In recent years, creative image editing has attracted substantial attention and seen significant advancements. Most recent works focus on how to modify the visible pixels in the image and have delivered impressive results, including image inpainting \citep{Xie_2023_CVPR}, composition \citep{yang2023paint} and colorization \citep{Chang_2023_CVPR}. However, assuming the image is a layered stack of objects and background, modifying images in the depth direction is less considered. In this paper, we investigate the object completion task which involves the restoration of partially occluded objects within an image (\cref{fig:teaser0}). By recovering the image to a stack of layered objects, a variety of depth-level editing can be developed. Unlike other conditional generation tasks, \eg, image inpainting, which only generates and integrates complete objects into images, object completion requires a seamless alignment between the generated content and the given partial object, which imposes more challenges to recover realistic and comprehensive object shapes.

In recent years, creative image editing has attracted substantial attention and seen significant advancements. Recent breakthroughs in image generation techniques have delivered impressive results across various image editing tasks, including image inpainting \citep{Xie_2023_CVPR}, composition \citep{yang2023paint} and colorization \citep{Chang_2023_CVPR}. However, another intriguing challenge lies in the domain of object completion (\cref{fig:teaser0}). This task involves the restoration of partially occluded objects within an image, representing the image as a layered stack of objects and background, which can potentially enable a number of more complicated editing tasks such as object layer switching. Unlike other conditional generation tasks, \eg, image inpainting, which only generates and integrates complete objects into images, object completion requires seamless alignment between the generated content and the given partial object, which imposes more challenges to recover realistic and comprehensive object shapes.
 
% Image segmentation revealing the shape of the objects has been demonstrated to have a close association with generation tasks. 
To guide the generative model in producing images according to a specific shape, additional conditions can be incorporated \citep{Koley_2023_CVPR,Yang_2023_CVPR}. Image segmentation has been shown to be a critical technique for enhancing the realism and stability of generative models by providing pixel-level guidance during the synthesis process. Recent research, as exemplified in the latest study by Zhang et al. \citep{zhang2023adding}, showcases that, by supplying object segmentations as additional high-quality masks for shaping the objects, it becomes possible to generate complex images of remarkable fidelity.

% insight why, double loop denoising (according to abs)

In this paper, we present MaskComp, a novel approach that bridges image generation and segmentation for effective object completion. MaskComp is rooted in a fundamental observation: the quality of the resulting image in the mask-conditioned generation is directly influenced by the quality of the conditioned mask \citep{zhang2023adding}. That says the more detailed the conditioned mask, the more realistic the generated image. 
Based on this observation, unlike prior object completion methods that solely rely on partially visible objects for generating complete objects, MaskComp introduces an additional mask condition combined with an iterative mask denoising (IMD) process, progressively refining the incomplete mask to provide comprehensive shape guidance to object completion.

Our approach formulates the partial mask as a noisy form of the complete mask and the IMD process is designed to iteratively denoise this noisy partial mask, eventually leading to the attainment of the complete mask. As illustrated in \cref{fig:teaser}, each IMD step comprises two crucial stages: generation and segmentation. The generation stage's objective is to produce complete object images conditioning on the visible portion of the target object and an object mask. Meanwhile, the segmentation stage is geared towards segmenting the object mask within the generated images and aggregating these segmented masks to obtain a superior mask that serves as the condition for the subsequent IMD step. By seamlessly integrating the generation and segmentation stages, we demonstrate that each IMD step effectively operates as a mask-denoising mechanism, taking a partially observed mask as input and yielding a progressively more complete mask as output. Consequently, through this iterative mask denoising process, the originally incomplete mask evolves into a satisfactory complete object mask, enabling the generation of complete objects guided by this refined mask.

The effectiveness of MaskComp is demonstrated by its capacity to address scenarios involving heavily occluded objects and its ability to generate realistic object representations through the utilization of mask guidance. In contrast to recent progress in the field of image generation research, our contributions can be succinctly outlined as follows:

\begin{itemize}
    \item We explore and unveil the benefits of incorporating object masks into the object completion task. A novel approach, MaskComp, is proposed to seamlessly bridge the generation and segmentation.
    
    \item We formulate the partial mask as a form of noisy complete mask and introduce an iterative mask denoising (IMD) process, consisting of alternating generation and segmentation stages, to refine the object mask and thus improve the object completion. 
    
    \item We conduct extensive experiments for analysis and comparison, the results of which indicate the strength and robustness of MaskComp against previous methods, \eg, Stable Diffusion. 
\end{itemize}

==> icml2024/src/2-related_works.tex <==
\section{Related Works}
\noindent\textbf{Conditional image generation.}
Conditional image generation \cite{lee2022autoregressive,gafni2022make,li2023gligen} involves the process of creating images based on specific conditions. These conditions can take various forms, such as layout \citep{li2020bachgan,sun2019image,zhao2019image}, sketch \citep{Koley_2023_CVPR}, or semantic masks \citep{gu2019mask}. For instance, Cascaded Diffusion Models \citep{ho2022cascaded} utilize ImageNet class labels as conditions, employing a two-stage pipeline of multiple diffusion models to generate high-resolution images. Meanwhile, in the work by \citep{sehwag2022generating}, diffusion models are guided to produce novel images from low-density regions within the data manifold. Another noteworthy approach is CLIP \citep{radford2021clip}, which has gained widespread adoption in guiding image generation in GANs using text prompts \citep{galatolo2021generating, gal2022stylegan, zhou2021lafite}. In the realm of diffusion models, Semantic Diffusion Guidance \citep{liu2023more} explores a unified framework for diffusion-based image generation with language, image, or multi-modal conditions. Dhariwal et al. \citep{dhariwal2021diffusion} employ an ablated diffusion model that utilizes the gradients of a classifier to guide the diffusion process, balancing diversity and fidelity. Furthermore, Ho et al. \citep{ho2022classifier} introduce classifier-free guidance in conditional diffusion models, incorporating score estimates from both a conditional diffusion model and a jointly trained unconditional diffusion model. 

\noindent\textbf{Object segmentation.}
In the realm of segmentation, traditional approaches have traditionally leaned on domain-specific network architectures to tackle various segmentation tasks, including semantic, instance, and panoptic segmentation \citep{fcn, deeplabv1, mask-rcnn, spatial-instance, associate-instance, solo, panoptic-deeplab, max-deeplab, li2023towards,li2023panoramic,li2023robust,li2023rethinking,li2023paintseg,li2022video,li2022hybrid}. However, recent strides in transformer-based methodologies, have highlighted the effectiveness of treating these tasks as mask classification challenges \citep{maskformer, knet, mask2former, detr}. MaskFormer \citep{maskformer} and its enhanced variant \citep{mask2former} have introduced transformer-based architectures, coupling each mask prediction with a learnable query. Unlike prior techniques that learn semantic labels at the pixel level, they directly link semantic labels with mask predictions through query-based prediction. Notably, the Segment Anything Model (SAM) \citep{kirillov2023segment} represents a cutting-edge segmentation model that accommodates diverse visual and textual cues for zero-shot object segmentation. Similarly, SEEM \citep{zou2023segment} is another universal segmentation model that extends its capabilities to include object referencing through audio and scribble inputs. By leveraging those foundation segmentation models, \eg, SAM and SEEM, a number of downstream tasks can be boosted \citep{ma2023segment,cen2023segment,yu2023inpaint}.




==> icml2024/src/3-method.tex <==
\section{MaskComp}
\label{sec:IMD}

\subsection{Problem Definition and Key Insight}
We address the object completion task, wherein the objective is to predict the image of a complete object $I_c\in\mathbb{R}^{3\times H\times W}$, based on its visible (non-occluded) part $I_p\in\mathbb{R}^{3\times H\times W}$. 
% Specifically, due to the ill-posed nature of this task, a language expression $E$ describing the appearance of the target object is also provided to facilitate the completion.

We first discuss the high-level idea of the proposed \textbf{I}terative \textbf{M}ask \textbf{D}enoising (IMD) and then illustrate the module details in \cref{sec:object completion} and \cref{sec:object segmentation}. The core of IMD is based on an essential observation: In the mask-conditioned generation, the quality of the generated object is intricately tied to the quality of the conditioned mask. As shown in \cref{fig:mask_condition}, we visualize the completion result of the same partial object but with different conditioning masks. We notice a more complete object mask condition will result in a more complete and realistic object image. 
Based on this observation, high-quality occluded object completion can be achieved by providing a complete object mask as the condition.

\begin{figure}[t]
% \hspace{-0.2cm}
\vspace{-0.2cm}
\includegraphics[width=\linewidth]{figs/mask_condition.pdf}
\vspace{-0.6cm}
\caption{Object completion with different mask conditions.}
\label{fig:mask_condition}
\vspace{-0.3cm}
\end{figure}

% Based on this observation, we propose the IMD process that effectively improves object completion by conducting a proxy task - mask denoising.

% (1) Unlike averaging generated object images, which can yield unrealistic and blurred results, averaging the generated object masks produces a more realistic and coherent shape. 
% (2) The quality of completed object is closely related to the conditioned mask. That says a more accurate conditioned mask can lead to a more reasonable completed object. 

\begin{figure*}[t]
    \centering    
    \includegraphics[width=\linewidth]{figs/pipeline.pdf}
    \vspace{-0.8cm}
    \caption{\textbf{Illustration of CompNet (generation stage of MaskComp).} The CompNet aims to recover the complete object $I_c$ from the partial object $I_p$ and a mask $M$. An object encoder is utilized to extract partial token $c_p$ which is gated and fed to the ControlNet to form the complete token $c_c$. The complete token $c_c$ serves as the condition to the diffusion U-Net to guide the conditional denoising process. In addition, a pre-diffusion mask is predicted from the partial token to encourage the object encoder to capture shape information.}
    % Given a complete object $I_c$ and its corresponding mask $M_c$, we first occlude the complete object and keep the visible part as $I_p$. Specifically, we sample a mask $M$ with an occlusion rate between visible and complete masks as the condition of the generative model during training.}
    % \ca{not mask, time embedding to alpha, augmented mask from complete img and partial img, occluded image not from complete image (explain where is partial image from and where is augmented image from), 
    % We do (1) mask augmentation, (2) object encoder, (3) gating, change encoder-decoder, controlnet to gray and ours blue,
    % segm as condition for image denoising, we need another pipeline for mask denoising (change figure 5 to this, (1) generate multiple instance, (2) segment, (3) fusing/voting/denoising, remove S(.), V(.))}
    % }
    \label{fig:pipeline}
\end{figure*}


% \ca{prob definition add figure, intuition add figure and then explain controlnet not work}
% \ca{why controlnet not work}
% \ca{mask denoising illustration}
% \ca{revise clarity of notations}
% \ca{two prob: image, mask, controlnet requires complete mask, but mask is not complete}
% \ca{overall intuition, iteratively mask better}
% \ca{painting for seg this inversed, two paper points seg + gen mutual benefit}
% \ca{use sam is because we explore the use of mask can benefit gen, we can add it to training but this is not our focus}
% \ca{add comparison to controlnet baseline, same data}
% \ca{change maskcomp name}
\subsection{Iterative Mask Denoising}
However, in real-world scenarios, the complete object mask is not available. To address this problem, we propose the IMD process which leverages intertwined generation and segmentation processes to approach the partial mask to the complete mask gradually. 
Given a partially visible object $I_p$ and its corresponding partial mask $M_p$, the conventional object completion task aims to find a generative model $\mathcal{G}$ such that $I_c\leftarrow\mathcal{G}(I_p)$, where $I_c$ is the complete object. Here, we additionally add the partial mask $M_p$ to the condition  $I_c\leftarrow\mathcal{G}(I_p, M_p)$, where $M_p$ can be assumed as an addition of the complete mask and a noise $M_p=M_c+\Delta$. By introducing a segmentation model $\mathcal{S}$, we can find a mask denoiser $\mathcal{S}\circ\mathcal{G}$ from the object completion model:
\begin{equation}
M_c\leftarrow\mathcal{S}\circ\mathcal{G}(I_p, M_c+\Delta)
\label{equ:mask denoiser}
\end{equation}
where $M_c=\mathcal{S}(I_c)$.
% In this way, we find a bridge to achieve more accurate mask estimation by generating more realistic images $I^*\leftarrow\mathcal{G}(I, M^*+\Delta)$.
% Empirically, we notice a better conditioned mask can lead to a better completed object
% \begin{equation}
%     \|I^*-\mathcal{G}(I, M^*+\Delta_1)\|_d<\|I^*-\mathcal{G}(I, M^*+\Delta_2)\|_d, \quad \text{if $\Delta_1<\Delta_2$}.
% \end{equation}
% where $\|\cdot\|_d$ is a distance function. Therefore, we can improve object completion by providing more accurate object masks.
% However, the complete object mask is not available as the target object is partially occluded. To address this problem, we introduce a segmentation model $\mathcal{S}$ to the object completion objective yielding a new target
% \begin{equation}
% M^*\leftarrow\mathcal{S}(\mathcal{G}(I, M^*+\Delta))
% \end{equation}
% which can be assumed as a mask-denoising process. 
% To conduct the mask denoising, we first train a generative model $\mathcal{G}$ to complete `the object with noisy mask guidance.
Starting from the visible mask $M_0=M_p$, as shown in \cref{fig:teaser}, we repeatedly apply the mask denoiser $\mathcal{S}\circ\mathcal{G}$ to gradually approach the visible mask $M_p$ to complete mask $M_c$. In each step, the input mask is denoised with a stack of generation and segmentation stages. Specifically, as the $\mathcal{S}\circ\mathcal{G}(\cdot)$ includes a generative process, we can obtain a set of estimations of denoised mask $\{M_t^{(k)}\}$. Here, we utilize a function $\mathcal{V}(\cdot)$ to find a more complete and reasonable mask from the $N$ sampled masks and leverage it as the input mask for the next iteration to further denoise. The updating rule can be written as:
\begin{equation}
M_{t}^{(k)}=\mathcal{S}\circ\mathcal{G}(I_p,\hat{M}_{t-1}),\,\,\,
\hat{M_t}=\mathcal{V}(M_t^{(1)},\cdots,M_t^{(N)})
\end{equation}
where $N$ is the number of sampled images in each iteration. With a satisfactory complete mask $\hat{M}_T$ after $T$ iterations, the object completion can be achieved accordingly by $\mathcal{G}(I_p,\hat{M}_T)$. The mathematical explanation of the process will be discussed in \cref{sec:discussion}. 

% In the IMD process, the denoised masks are first generated by the stack of segmentation and generation models $\mathcal{S}(\mathcal{G}(\cdot))$, and then its expectation is estimated by the averaging operation. 


% Let us denote the occluded object mask as $M+\Delta$ where $M$ is the complete object mask and the $\Delta$ is the mask noise. Mask denoising aims to find a function $\mathcal{F}$ that makes $\mathcal{F}(M+\Delta)=M$. In OCMD, we utilize a conditional generation $\mathcal{G}$ and a segmentation $\mathcal{S}$ module to model the function $\mathcal{F}$ as $\mathcal{S}(\mathcal{G}(M+\Delta))=M$. The process first generates images by taking the object masks as conditions and then segments them to estimate masks. Specifically, if we assume the segmentation module $\mathcal{S}$ is perfect, we can rewrite the target as

% SegComp leverages the progressive masked revision (PMR) to gradually complete and refine the partially occluded object $I_p$. The PMR process is composed of alternating G-step (Generation) and S-step (Segmentation), as illustrated in Figure~\ref{fig:teaser}. During G-step, a more complete object $I_c^t=\mathcal{D}(I_p, M^t)$ is generated with a diffusion-based generative model $\mathcal{D}(\cdot)$ conditioned on the non-occluded part of the object $I_p$ and an object mask $M^t$. During S-step, the object mask $M^{t+1}=\mathcal{B}(I_c^t, \mathcal{S})$ is achieved by a Bayesian estimation method $\mathcal{B}$ with a segmentation model $\mathcal{S}$ and the generated image $I_c^t$ from G-step. With the alternating the G-steps and S-steps, the generated object can be gradually advanced.

% Here, the amodal image $I_c$ and amodal mask $M_{a}$ serve as the proxy to bridge the segmentation and completion. By alternating C-step and S-step, the ICR process performs in an expectation–maximization-like (EM-like) manner. As the formulation is symmetry, both $I_c$ and $M_{a}$ can be considered as the latent variable of the EM-like process. Specifically, $I_c$ can be assumed as the latent variable for amodal segmentation and $M_{a}$ for amodal completion. 

\subsection{Generation Stage}
\label{sec:object completion}
We introduce \textbf{\textsl{CompNet}} as the generative model $\mathcal{G}$ which aims to recover complete objects based on partial conditions. We build CompNet based on popular ControlNet \cite{zhang2023adding} while making fundamental modifications to enable object completion. As shown in \cref{tab:form diff}, the target of ControlNet is to generate images strictly based on the given conditions, \ie, $I_p\leftarrow\mathcal{G}(I_p,M_p)$, making it unable to complete object. Differently, CompNet is designed to recover the object. With a segmentation network, it can act as a mask denoiser to refine the conditioned mask, \ie, $M_c\leftarrow\mathcal{S}\circ\mathcal{G}(I_p,M_p)$.

\begin{table}[t]
    \centering
    \scalebox{0.77}{
    \begin{tabular}{c|ccc}
    \hline
    Method  & Objective & Objective with Segm. &  Object Comp.\\
    \hline
    ControlNet & $I_p\leftarrow\mathcal{G}(I_p,M_p)$ & $M_p\leftarrow\mathcal{S}\circ\mathcal{G}(I_p,M_p)$ & \textcolor{red}{\XSolidBrush}\\
    CompNet & $I_c\leftarrow\mathcal{G}(I_p,M_p)$ & $M_c\leftarrow\mathcal{S}\circ\mathcal{G}(I_p,M_p)$ & \textcolor{mygreen}{\Checkmark}\\
    \hline
    \end{tabular}}
    \vspace{-0.2cm}
    \caption{Objective difference with ControlNet.}
    \label{tab:form diff}
    \vspace{-0.8cm}
\end{table}

\noindent\textbf{Mask condition.}
% As shown in left of the \cref{fig:pipeline}, given a complete object $I_c$ and its corresponding mask $M_c$, we first occlude the complete object and keep the partially visible part as $I_p$. Recall that the mask-denoising process starts from the partial mask $M_p$ and ends at the complete mask $M_c$. To enable iterative denoising, the model should be able to tackle any mask between the input partial and the output complete mask. Therein, during training, we sample a mask $M$ from the interpolations between the partial and complete mask as the condition of the generative model. 
As illustrated on the left side of \cref{fig:pipeline}, we begin with a complete object $I_c$ and its corresponding mask $M_c$. Our approach commences by occluding the complete object, retaining only the partially visible portion as $I_p$. Recall that the mask-denoising procedure initiates with the partial mask $M_p$ and culminates with the complete mask $M_c$. To facilitate this iterative denoising, the model must effectively handle any mask that falls within the interpolation between the initial partial mask and the target complete mask. Consequently, we introduce a mask $M$ with an occlusion rate positioned between the partial and complete masks as a conditioning factor for the generative model. During training, we conduct the random occlusion process (detailed in Appendix C) twice for each complete mask $M_c$. The partial mask $M_p$ is achieved by considering the occluded areas in both occlusion processes. The interpolated mask $M$ is generated by using one of the occlusions. 

\noindent\textbf{Diffusion model.}
Diffusion models have achieved notable progress in synthesizing unprecedented image quality and have been successfully applied to many text-based image generation works \citep{rombach2022high,zhang2023adding}. For our object completion task, the complete object can be generated by leveraging the diffusion process.

Specifically, the diffusion model generates image latent $x$ by gradually reversing a Markov forward process. As shown in Figure~\ref{fig:pipeline}, starting from $x_0=\mathcal{E}(I_c)$, the forward process yields a sequence of increasing noisy tokens $\{x_\tau|\tau\in[1,T_{\mathcal{G}}]\}$, where $x_\tau=\sqrt{\Bar{\alpha_\tau}}y_0+\sqrt{1-\Bar{\alpha_\tau}}\epsilon$, $\epsilon$ is the Gaussian noise, and $\alpha_\tau$ decreases with the timestep $\tau$. For the denoising process, the diffusion model progressively denoises a noisy token from the last step given the conditions $c=(I_p,M,E)$ by minimizing the following loss function: $\mathcal{L}=\mathbb{E}_{\tau,x_0,\epsilon}\|\epsilon_\theta(x_\tau,c,\tau)-\epsilon\|_2^2$. $I_p$, $M$, and $E$ are the partial object, conditioned mask, and text prompt respectively.
% More details about the diffusion process are available in the Appendix.
\begin{figure*}[t]
    \centering    
    \includegraphics[width=\linewidth]{figs/mask.pdf}
    \vspace{-0.7cm}
    \caption{
    % (a) Illustration of the segmentation stage. (b) Visualization of the probability of mask. 
    We calculate the mask probability map by averaging and normalizing the masks of sampled images. We show a cross-section of the lower leg to better visualize (shown as \textcolor{darkyellow}{yellow}). 
    }
    \vspace{-0.3cm}
    \label{fig:mask}
\end{figure*}

\noindent\textbf{CompNet architecture.}
Previous work \citep{zhang2023adding} has demonstrated an effective way to add additional control to generative diffusion models. We follow this architecture and make necessary modifications to adapt the architecture to object completion. As shown in \cref{fig:pipeline}, given the visible object $I_p$ and the conditioning mask $M$, we first concatenate them and extract the partial token $c_p$ with an object encoder. 
% After that, we learn an object controller to add additional conditions to the network. 
Different from ControlNet \citep{zhang2023adding} assuming the condition is accurate, the object completion task relies on incomplete conditions. Specifically, in the early diffusion steps, the condition information is vital to complete the object. Nevertheless, in the later steps, inaccurate information in the condition can degrade the generated object. To tackle this problem, we introduce a time-variant gating operation to adjust the importance of conditions in the diffusion steps. We learn a linear transform $f: \mathbb{R}^{C}\rightarrow\mathbb{R}^{1}$ upon the time embedding $e_t\in\mathbb{R}^{C}$ and then apply it to the partial token as $f(e_t)\cdot c_p$ before feeding it to the ControlNet. In this way, the importance of visible features can be adjusted as the diffusion steps forward. The time embedding used for the gating operation is shared with the time embedding for encoding the diffusion step in the stable diffusion.

To encourage the object encoder to capture shape information, we introduce an auxiliary path to predict the complete object mask from the partial token $c_p$. Specifically, a feature pyramid network \cite{lin2017feature} is leveraged as the mask decoder which takes $c_p$ and the multi-scale features from the object encoder as input and outputs a pre-diffusion mask $M_{pre}$. We encourage mask completion with supervision as
\begin{equation}
    \mathcal{L}_{mask}=\mathcal{L}_{dice}(M_c,M_{pre})+\lambda_{ce}\mathcal{L}_{ce}(M_c,M_{pre})
\end{equation}
where $\mathcal{L}_{dice}$ and $\mathcal{L}{ce}$ are Dice loss \cite{li2019dice} and BCE loss respectively. $\lambda_{ce}$ is a constant.

\subsection{Segmentation Stage}
\label{sec:object segmentation}
In the segmentation stage, illustrated in \cref{fig:mask} (a), our approach initiates by sampling $N$ images denoted as $\{I_t^{(k)}\}^N_{k=1}$ from the generative model, where $t$ is the IMD step. Subsequently, we employ an off-the-shelf object segmentation model denoted as $\mathcal{S}(\cdot)$ to obtain the shapes (object masks) $\{M_t^{(k)}\}$ from these sampled images.

To derive an improved mask for the subsequent IMD step, we seek a function $\mathcal{V}(\cdot)$ that can produce a high-quality mask prediction from the set of $N$ generated masks. Interestingly, though the distribution of sampled images is complex, we notice the distribution of masks has good properties.
In \cref{fig:mask} (b), we provide a visualization of the probability map associated with a set of object masks with the same conditions, which is computed by taking the normalized average of the masks.
% as $p(M)[i,j]=\frac{\sum_{i=1}^N M^{(i)}[i,j]}{N}$ where $[i,j]$ is the coordinate of a pixel in the mask. 
% Notably, we observe that this mask probability map tends to exhibit an unimodal and symmetric property which makes it feasible to maximize the mask probability by voting.
% , facilitating the identification of high-probability regions.
% Interestingly, we realize that the mask probability approximately follows an unimodal distribution which makes it easy to discriminate high-probability regions. 
% To better visualize the probability, we pick a cross-section of the fully occluded part in $I_p$ (lower leg, shown as {\color{yellow}{yellow}} section) and visualize the probability with respect to the horizontal coordinate.
To enhance the visualization of this probability distribution, we focus on a specific cross-section of the fully occluded portion in image $I_p$ (the lower leg, represented as a \textcolor{darkyellow}{yellow} section) and visualize the probability as a function of the horizontal coordinate which demonstrates an obvious unimodal and symmetric property. Leveraging this observation, we can find an improved mask by taking the high-probability region. 
% The updating rule can be derived as 
% \begin{equation}
%     \hat{M}_t=\frac{\sum_{i=1}^NM_t^{(i)}}{N}
% \end{equation}
% where $N$ is the number of sampled masks.
The updating can be achieved by conducting a voting process across the $N$ estimated masks, as defined by the following equation:
\begin{equation}
    \hat{M}_t[i,j] = \begin{cases}
                1, & \text{if}\quad \frac{\sum_{k=1}^NM_t^{(k)}[i,j]}{N} \geq \tau \\
                0, & \text{otherwise}
        \end{cases}
\end{equation}
where $[i,j]$ denotes the coordinate, and $\tau$ is the threshold employed for the mask voting process.
% Note that, as the randomness only lies in the generative diffusion model, the $\mathcal{S}$ can be assumed as a non-linear transform applied to the sampled images. As discussed in Section \ref{sec:mask as a bridge}, the expectation of generated image $\mathbb{E}[I_c]$ is suboptimal as the image distribution is complicated thus the expectation can fall in the low-probability regions leading to unrealistic. To solve this problem, we leverage a segmentation model to project the image to the mask space which we empirically find that the distribution $p(M|I_p)$ is unimodal and symmetric. Therein, the expectation $\mathbb{E}[M]$ can be meaningful and realistic.
% As discussed in Section \ref{sec:mask as a bridge}, to make the $\mathbb{E}[\mathcal{S}(I_c)]$ reasonable, it is necessary to ensure $p(\mathcal{S}(I_c)|I_p)$ to be unimodal and symmetric. 




% object completion as a mask diffusion, mask diffusion = image diffusion + segmentation model

% image diffusion and mask diffusion compare

% image diffusion estimate noise in each step

% mask diffusion estimates what in each step

% Image:
% training: I+delta = delta
% noise is explicitly computed, gaussian noise
% inference: sampling, added to the image

% Mask:
% training: noise mask, manually added noise, cut mask (this is the same as diffusion)

% inference (this is different): sample but don't know how to add, sample multiple image fuse

% combine image diffusion and mask diffusion:
% two loops, inner image diffusion, outer mask diffusion

% draw a figure:
% image gen: img diff

% obj completion: img diff + mask diff

% comparison

\begin{figure}[t]
\centering   
\includegraphics[width=\linewidth]{figs/dist.pdf}
\vspace{-0.8cm}
\caption{\textbf{Mutual-benificial sampling.}}
\vspace{-0.5cm}
\label{fig:mutual}
\end{figure}

\begin{table*}[t]
\centering
\scalebox{0.9}{
\begin{tabular}{l|p{1.4cm}<{\centering}p{1.4cm}<{\centering}p{1.4cm}<{\centering}p{1.4cm}<{\centering}|p{1.4cm}<{\centering}p{1.4cm}<{\centering}p{1.4cm}<{\centering}p{1.4cm}<{\centering}} 
\hline
\multirow{2}*{Method} & \multicolumn{4}{c|}{AHP \citep{zhou2021human}} &
\multicolumn{4}{c}{DYCE \citep{ehsani2018segan}}\\
\cline{2-9}
~ & FID-G $\downarrow$ & FID-S $\downarrow$ & Rank $\downarrow$ & Best $\uparrow$ & FID-G $\downarrow$ & FID-S $\downarrow$ & Rank $\downarrow$ & Best $\uparrow$\\
\hline
ControlNet & 40.2 & 45.4 & 3.4 & 0.10 & 42.4 & 49.4 & 3.4 & 0.08 \\
Kandinsky 2.1 & 43.9 & 39.2 & 3.2 & 0.11 & 44.3 & 47.7 &  3.4 & 0.06 \\
Stable Diffusion 1.5 & 35.7 & 41.4 & 3.2 & 0.12 & 31.2 & 43.4 & 3.4 & 0.11 \\
Stable Diffusion 2.1 & 30.8 & 39.9 & 3.1 & 0.14 & 30.0 & 41.1 & 3.0 & 0.12 \\
\bf MaskComp (Ours) & \bf16.9 & \bf21.3 &\bf2.1 & \bf0.53 & \bf 20.0 & \bf25.4 & \bf1.9 & \bf0.63  \\
\hline
\end{tabular}}
\caption{\textbf{Quantitative evaluation on object completion task}. The computing of FID-G and FID-S only considers the object areas within ground truth and foreground regions segmented by SAM, respectively, to eliminate the influence of the generated background. The Rank denotes the average ranking in the user study. The Best denotes the percentage of samples that are ranked as the best. $\downarrow$ and $\uparrow$ denote the smaller the better and the larger the better respectively.}
\label{tab:main results}
\vspace{-0.3cm}
\end{table*}

\subsection{Discussion}
\label{sec:discussion}
% In this section, we discuss the mathematical explanation of MaskComp, where we will omit the conditioned partial image $I_p$ for simplicity.
In this section, we will omit the conditioned partial image $I_p$ for simplicity.

\noindent\textbf{Joint modeling of mask and object.}
In practical scenarios where the complete object mask $M_c$ is unavailable, modeling object completion through a marginal probability $p(I_c|M_c)$ becomes infeasible. Instead, it necessitates the more challenging joint modeling of objects and masks, denoted as $p(I,M)$, where the images and masks can range from partial to complete. Let us understand the joint distribution by exploring its marginals. Since the relation between mask and image is one-to-many (each object image only has one mask while the same mask can be segmented from multiple images), the $p(M|I)$ is actually a Dirac delta distribution $\delta$ and only the $p(I|M)$ is a real distribution. This way, the joint distribution of mask and image is discrete and complex, making the modeling difficult. To address this issue, we introduce a slack condition to the joint distribution $p(I,M)$ that \textit{the mask and image can follow a many-to-many relation}, which makes its marginal $p(M|I)$ a real distribution and permits $p(I|M)$ to predict image $I$ that has a different shape as the conditioned $M$ and vice versa. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/compare.pdf}
    \vspace{-0.7cm}
    \caption{\textbf{Qualitative comparison against ControlNet, Kandinsky and Stable Diffusion}. The background is filtered out for better visualization. More results are available in the Appendix.}
    \label{fig:compare}
\end{figure*}

\noindent\textbf{Mutual-beneficial sampling.}
After discussing the joint distribution that we are targeting, we introduce the mathematical explanation of MaskComp. MaskComp introduces the alternating modeling of two marginal distributions $p(I|M)$ (generation stage) and $p(M|I)$ (segmentation stage), which is actually a Markov Chain Monte Carlo-like (MCMC-like) process and more specifically Gibbs sampling-like. It samples the joint distribution $p(I,M)$ by iterative sampling from the marginal distributions. Two core insights are incorporated in MaskComp: (1) providing a mask as a condition can effectively enhance object generation and (2) fusing the mask of generated object images can result in a more accurate and complete object mask. Based on these insights, we train CompNet to maximize $p(I|M)$ and leverage mask voting to maximize the $p(M|I)$. As shown in \cref{fig:mutual}, MaskComp develops a mutual-beneficial sampling process from the joint distribution $p(I,M)$, where the object mask is provided to boost the image generation and, in return, the generated images can lead to a more accurate mask by fusing the segmentation of images. Through alternating sampling from the marginal distributions, we can effectively address the object completion task.


==> icml2024/src/4-experiment.tex <==
\section{Experiment}
\subsection{Experimental Settings}
\noindent\textbf{Dataset.}
We evaluate MaskComp on two popular datasets: AHP \citep{zhou2021human} and DYCE \citep{ehsani2018segan}. 
% COCOA is a dataset for amodal object segmentation which contains 2,476 training images and 1,223 testing images within 80 instance classes about common objects. Specifically, COCOA augments each object with an amodal mask to describe the shape of the occluded part. 
AHP is an amodal human perception dataset with 56,302 images with annotations of integrated humans.
% that is composed of a training set with 56,302 images with annotations of integrated humans, a validation set with 297 images of synthesized occlusion cases, and a test set with 56 images of artificial occlusion cases. 
% As the original test split is too small, we resplit 10,000 images from the training set for evaluation. 
DYCE is a synthetic dataset with photo-realistic images and the natural configuration of objects in indoor scenes.
% 41,924 and 27,617 objects are involved in the training set and test sets respectively. 
For both datasets, the non-occluded object and its corresponding mask for each object are available. We train MaskComp on the AHP and a filtered subset of OpenImage v6 \citep{kuznetsova2020open}. OpenImage is a large-scale dataset offering heterogeneous annotations. We select a subset of OpenImage that contains 429,358 objects as a training set of MaskComp.


\tableablation{t}

\noindent\textbf{Evaluation metrics.}
In accordance with previous methods \citep{zhou2021human}, we evaluate image generation quality Fréchet Inception Distance (FID). The background is removed with object masks before evaluation. 
As the FID score cannot reflect the object completeness, we further conduct a user study, leveraging human assessment to compare the quality and completeness of images. During the assessment, given a partial object, the participants are required to rank the generated object from different methods based on their completeness and quality. We calculate the averaged ranking and the percentage of the image being ranked as the first place as the metrics (details available in the Appendix).

\noindent\textbf{Implementation details.}
For the generation stage, we train the CompNet with frozen Stable Diffusion \citep{rombach2022high} on the AHP dataset for 50 epochs. The learning rate is set for 1e-5. We adopt $\mathrm{batchsize}=8$ and an Adam \citep{loshchilov2017adamw} optimizer. 
The image is resized to $512\times 512$ for both training and inference. 
The object is cropped and resized to have the longest side 360 before sticking on the image. 
% We follow \citep{zhang2023adding} to occlude objects. 
For a more generalized setting, we train the CompNet on a subset of the OpenImage \citep{kuznetsova2020open} dataset for 36 epochs. We generate text prompts using BLIP \citep{li2022blip} for all experiments (prompts are necessary to train ControlNet). For the segmentation stage, we leverage SAM \citep{kirillov2023segment} as $\mathcal{S}(\cdot)$. We vote mask with a threshold of $\tau=0.5$. During inference, if no other specification, we conduct the IMD process for 5 steps with $N=5$ images for each step. We give the class label as the text prompt to facilitate the CompNet to effectively generate objects. All baseline methods are given the same text prompts during the experiments. More implementation details are available in the appendix. The code will be made publicly available.

\subsection{Main Results}

\noindent\textbf{Quantitative results.}
We compare the MaskComp with state-of-the-art methods, ControlNet \citep{zhang2023adding}, Kandinsky 2.1 \citep{kandinsky2}, Stable Diffusion 1.5 \citep{rombach2022high} and Stable Diffusion 2.1 \citep{rombach2022high} on AHP \citep{zhou2021human} and DYCE \citep{ehsani2018segan} dataset. The results in \cref{tab:main results} indicate that MaskComp consistently outperforms other methods, as evidenced by its notably lower FID scores, signifying the superior quality of its generated content. We conducted a user study to evaluate object completeness in which participants ranked images generated by different approaches. MaskComp achieved an impressive average ranking of 2.1 and 1.9 on the AHP and DYCE datasets respectively. Furthermore, MaskComp also generates the highest number of images ranked as the most complete and realistic compared to previous methods. We consider the introduced mask condition and the proposed IMD process benefits the performance of MaskComp, where the additional conditioned mask provides robust shape guidance to the generation process and the proposed iterative mask denoising process refines the initial conditioned mask to a more complete shape, further enhancing the generated image quality.   

\noindent\textbf{Qualitative results.}
We present visual comparisons among ControlNet, Kandinsky 2.1, Stable Diffusion 1.5, and Stable Diffusion 2.1, illustrated in \cref{fig:compare}. Our visualizations showcase MaskComp's ability to produce realistic and complete object images given partial images as the condition, whereas previous approaches exhibit noticeable artifacts and struggle to achieve realistic object completion. In addition, without mask guidance, it is common for previous methods to generate images that fail to align with the partial object.

\begin{figure*}[t]
    \centering    
    \vspace{-0.1cm}
    \includegraphics[width=\linewidth]{figs/vis_imd.pdf}
    \vspace{-0.65cm}
    \caption{\textbf{Visualization of the IMD process.} For each step, we randomly demonstrate one generated image and the averaged mask for all generated images. We omit the input mask which has the same shape as the input occluded object.
    }
    \label{fig:vis_imd}
    % \vspace{-0.1cm}
\end{figure*}

\tabdesignchoice{t}

\subsection{Analysis}
\label{sec:analysis}
In this section, we provide an experimental analysis of MaskComp. All the results are evaluated with GT masks to filter out the background, \ie, FID-G.

\noindent\textbf{Performance with different mask conditions.}
We evaluated the quality of generated images when conditioned on the same partial images along with three distinct types of masks: (1) partial mask (mask of the partial image), (2) intermediate mask (less occlusion than partial), and (3) complete mask. As shown in \cref{tab:conditioned mask}, the model achieves its highest performance when it is conditioned with complete object masks, whereas relying solely on partial masks yields less optimal results. These results provide strong evidence that the quality of the conditioned mask significantly influences the quality of the generated images.

\noindent\textbf{Performance with different occlusion rates.}
We perform ablation studies to assess the resilience of MaskComp under varying occlusion levels. As presented in \cref{tab:occ}, we evaluate MaskComp at different occlusion levels (proportion of the obscured area relative to the complete object) ranging from 20\% to 80\%, and the results indicate that its performance does not degrade significantly up to 60\% occlusion.
% Even at 60\% occlusion rates, its robust performance holds up. 
% However, a further increase in the occlusion rate to an extreme level will result in MaskComp not producing high-quality images.
% These experimental results underscore the robustness of MaskComp, even when confronted with significantly occluded objects.

% \noindent\textbf{Inference speed.}
% do not mention
% We provide the inference speed breakdown for each step of IMD, as presented in \cref{tab:}. We observe that the generative diffusion step consumes the majority of computation time, while the remaining components require only a fraction of the total processing time.

% \noindent\textbf{Performance without complete object during training.}
% Occlusion is a prevalent occurrence in images, posing a significant challenge for object completion, primarily due to the unavailability of ground-truth complete objects. This motivates us to investigate the performance of MaskComp without ground-truth complete objects during training. As MaskComp relies on a mask denoising process that does not necessarily request the complete objects during training (a detailed analysis available in Appendix A), it is possible to adapt MaskComp to the scenarios without complete objects available during training. As shown in \cref{tab:comp obj}, we report the performance on AHP dataset with the models trained on AHP (with complete objects) and OpenImage (without complete objects) respectively. We notice that the performance of MaskComp trained on OpenImage is just slightly lower than that trained with AHP dataset, indicating that MaskComp has the potential to be adapted to the scenarios without ground-truth complete objects. More qualitative comparisons are available in the Appendix.


\noindent\textbf{Inference time.} \cref{tab:time} reports the inference time of each component in IMD (with a single NVIDIA V100 GPU). Although MaskComp's throughput is reduced due to the inclusion of multiple diffusion processes in each IMD step, it is capable of attaining a higher degree of accuracy in visual object completion. Based on our empirical experiments, reducing the number of diffusion steps during the first few IMD steps can increase model speed without sacrificing much performance. With this idea incorporated into MaskComp, the average running time could be reduced to 2/3 of the original time with FID slightly increasing by 0.50. While beyond the scope of this study, we expect more advanced techniques could be explored to optimize the tradeoff between model speed and performance.

\noindent\textbf{Comparison to amodal segmentation baseline.}
Amodal segmentation has a similar objective to the proposed IMD process. To demonstrate the effectiveness of MaskComp, we construct an amodal baseline that generates amodal masks from the SOTA amodal segmentation method \cite{tran2022aisformer} and then utilize ControlNet to generate images based on the amodal masks. s shown in \cref{tab:amodal}, we notice that our method outperforms the amodal baseline by a considerable margin, which could be attributed to the strong mask completion capability of the proposed IMD process.
% \ca{We demonstrate the inference time of each component in IMD as shown in \cref{tab:time} (with a single NVIDIA V100 GPU). Due to the multiple diffusion processes in each IMD step, the inference speed of MaskComp is slow. To improve the inference speed, we notice that decreasing the diffusion step number in the first several IMD steps will not severely degrade the performance. By incorporating this idea into MaskComp, the average running time was reduced to 2/3 original time with a slight FID increase of 0.5.}

\begin{table}[t]
    \centering
    \scalebox{0.95}{
    \begin{tabular}{c|ccccc}
        Noise degree & Iter. 1 & Iter. 3 & Iter. 5 & Iter. 7 & Iter. 9 \\
        \toprule
        15\% area & 28.4 & 22.7 & 18.9 & 17.2 & 16.5 \\
        10\% area & 26.4 & 21.4 & 18.1 & 17.0 & 16.4 \\
        5\% area & 24.9 & 19.6 & 17.0 & 16.2 & 16.0 \\
        No noise & 24.7 & 19.4 & 16.9 & 16.1 & 15.9 
    \end{tabular}}
    \vspace{-0.2cm}
    \caption{Performance against segmentation errors on AHP dataset.}
    \vspace{-0.3cm}
    \label{tab:robust}
\end{table}

\noindent\textbf{Impact of different segmentation networks.} 
We adopt SAM to obtain object masks at the segmentation stage. To study the impacts of different segmenters, we replace SAM with two smaller segmentation networks, CLIPSeg \cite{luddecke2022image} and SEEM \cite{zou2023segment}. \cref{tab:segm model} shows that the FID score with CLIPSeg (19.9) is slightly higher than with SAM (16.9), but remains competitive against other state-of-the-art methods, e.g., Stable Diffusion 2.1 (30.8 reported in \cref{tab:main results}). MaskComp is an iterative mask denoising (IMD) process that progressively refines a partial object mask to boost image generation. The results support our hypothesis that the impact of the segmenter is modest.

% \CC{Q: Line 426. 30.8 is FID-G from Table 2. Does FID-G use object ground truth, not SAM? }


\noindent\textbf{Design choices in IMD.}
We conduct experiments to ablate the design choices in IMD and their impacts on the completion performance. We first study the effect of IMD step number. With a larger step number, IMD can better advance the partial mask to the complete mask. As shown in \cref{tab:step number}, we notice that the image quality keeps increasing and slows down at a step number of 5. In this way, we choose 5 as our IMD step number. After that, we ablate the number of sampled images in the segmentation stage in \cref{tab:image number}. We notice more sampled images generally leading to a better performance. We leverage an image number of 5 with the efficiency consideration. As we leverage the diffusion-based method for image generation, we ablate the iterations for the diffusion process. As shown in \cref{tab:gating}, we notice the gating operation improves the generation quality by 1.3 FID, indicating the necessity of conditional gating.


\noindent\textbf{Robustness to segmentation errors.} 
We conduct experiments to manually add random errors to masks. As shown in \cref{tab:robust}, we ablate on the number of iterations and the degree of segmentation error. We observe that segmentation errors will increase the convergence iteration number while not affecting the final performance significantly. As IMD is a reciprocal process intended to provide effective control for later-generated masks to be refined based on adaptive feedback, mask errors are mitigated and not propagated.


\noindent\textbf{Visualization of iterative mask denoising.}
To provide a clearer depiction of the IMD process, as depicted in \cref{fig:vis_imd}, we present visualizations of the generated image and the averaged mask for each step. In the initial step, we observe the emergence of artifacts alongside the object. As we progress through the steps, both the image and mask quality exhibit continuous improvement.

% More results and analysis are available in the Appendix.






==> icml2024/src/5-conclusion.tex <==
% \vspace{0.05cm}
\section{Conclusion}
In this paper, we introduce MaskComp, a novel approach for object completion. MaskComp addresses the object completion task by seamlessly integrating conditional generation and segmentation, capitalizing on the crucial observation that the quality of generated objects is intricately tied to the quality of the conditioned masks. We augment the object completion process with an additional mask condition and propose an iterative mask denoising (IMD) process. This iterative approach gradually refines the partial object mask, ultimately leading to the generation of satisfactory objects by leveraging the complete mask as a guiding condition. Our extensive experiments demonstrate the robustness and effectiveness of MaskComp, particularly in challenging scenarios involving heavily occluded objects.

% \noindent\textbf{Limitations.}
% As shown in \cref{tab:occ}, MaskComp faces challenges in scenarios where the occlusion rate is exceedingly high, making it difficult to recognize the conditioned content and resulting in the failure to generate realistic complete objects. Addressing situations of high occlusion, we consider additional guidance essential to further refine the object completion process.


% occlusion rate is super big still fail
% add failure case in supp, cannot recognize the content (refer to)
% While MaskComp excels at robustly completing partial objects through the IMD process, it entails higher computational demands compared to prior methods, primarily due to its iterative nature. We observed that the convergence speed is tied to the generation ability at each step. Therefore, with the development of stronger generative models in the future, it may be possible to further streamline the steps involved in MaskComp.



==> icml2024/src/tables.tex <==
\def\tabdesignchoice#1{
\begin{table*}[#1]
	\centering
 	\subfloat[
	\textbf{Segmentation model}.
	\label{tab:segm model}
	]{
		\begin{minipage}{0.25\linewidth}{\begin{center}
					\tablestyle{1.5pt}{1.2}
					\begin{tabular}{l|ccc}
                        % \shline
                        Model & CLIPSeg & SEEM & SAM \\ [.1em]
                        \shline
					FID & 19.9 & 18.1 & 16.9\\
                        % \hline
                    \end{tabular}
		\end{center}}\end{minipage}
	}
	\subfloat[
	\textbf{IMD step number}.
	\label{tab:step number}
	]{
		\begin{minipage}{0.25\linewidth}{\begin{center}
    \tablestyle{1.5pt}{1.2}
    \begin{tabular}{l|ccccc}
        % \shline
        $T$ & 1 & 3 & 5 & 7 \\ [.1em]
        \shline
        FID & 24.7 & 19.4 & 16.9 & 16.1  \\
        % \hline
    \end{tabular}
\end{center}}\end{minipage}
}
\subfloat[
	\textbf{\# of sampled images}.
	\label{tab:image number}
	]{
		\centering
		\begin{minipage}{0.25\linewidth}{\begin{center}
    \tablestyle{1.5pt}{1.2}
    \begin{tabular}{l|ccc}
        % \shline
        N & 4 & 5 & 6 \\ [.1em]
        \shline
    FID & 17.4 & 16.9 & 16.8 \\
        % \hline
    \end{tabular}
		\end{center}}\end{minipage}
	}
    \subfloat[
	\textbf{Condition gating}.
	\label{tab:gating}
	]{
		\begin{minipage}{0.2\linewidth}{\begin{center}
					\tablestyle{1.5pt}{1.2}
					\begin{tabular}{l|cccc}
                        % \shline
                        Gating & \Checkmark & \XSolidBrush \\ [.1em]
                        \shline
						FID & 16.9 & 18.2\\
                        % \hline
                    \end{tabular}
		\end{center}}\end{minipage}
	}
 \vspace{-0.1cm}
	\caption{\textbf{Design choices for IMD on AHP dataset.} We ablate (a) the impact of different segmentation networks, (b) IMD step number, (c) the number of sampled images in the segmentation stage, and (d) the gating operation in the CompNet.}
    \vspace{-0.2cm}
	\label{tab:design choices}
\end{table*}}


\def\tableablation#1{
\begin{table*}[#1]
	\centering
	\subfloat[
	\textbf{Conditioned mask}.
	\label{tab:conditioned mask}
	]{
		\begin{minipage}{0.25\linewidth}{\begin{center}
    \tablestyle{1.5pt}{1.2}
    \begin{tabular}{l|ccccc}
        % \shline
        Mask & Partial & Intermed. & Complete \\ [.1em]
        \shline
        FID & 16.9 & 15.3 & 12.7   \\
        % \hline
    \end{tabular}
\end{center}}\end{minipage}
}
	\subfloat[
	\textbf{Occlusion rate}.
	\label{tab:occ}
	]{
		\begin{minipage}{0.27\linewidth}{\begin{center}
					\tablestyle{1.5pt}{1.2}
					\begin{tabular}{l|cccc}
                        % \shline
                        Occ. & 20\% & 40 \% & 60 \% & 80\%\\ [.1em]
                        \shline
					FID & 13.4 & 15.7 & 17.2 & 29.9\\
                        % \hline
                    \end{tabular}
		\end{center}}\end{minipage}
	}
 \subfloat[
	\textbf{Inference time}.
	\label{tab:time}
	]{
		\centering
		\begin{minipage}{0.2\linewidth}{\begin{center}
    \tablestyle{1.5pt}{1.2}
    \begin{tabular}{l|ccc}
        % \shline
        Comp. & Gen. & Segm. & Total \\ [.1em]
        \shline
    Second &  14.3 & 1.2 & 15.5 \\
        % \hline
    \end{tabular}
		\end{center}}\end{minipage}
	}
  \subfloat[
	\textbf{Amodal baseline}.
	\label{tab:amodal}
	]{
		\centering
		\begin{minipage}{0.25\linewidth}{\begin{center}
    \tablestyle{1.5pt}{1.2}
    \begin{tabular}{l|ccc}
        % \shline
        Model & Baseline & MaskComp \\ [.1em]
        \shline
    FID & 29.4 & 16.9 \\
        % \hline
    \end{tabular}
		\end{center}}\end{minipage}
	}
 \vspace{-0.1cm}
	\caption{\textbf{Ablation of MaskComp on AHP dataset}. We ablate (a) the different conditioning masks during inference, (b) the occlusion rate during inference, (c) the inference time of each component in an IMD step, and (d) the performance compared with the amodal baseline.}
 % (c) We report the performance of MaskComp trained with or without the complete objects.}
	\label{tab:ablation}
\end{table*}}


\def\tablemoreablation#1{
\begin{table*}[#1]
	\centering
	\subfloat[
	\textbf{Iteration for diffusion}.
	\label{tab:iter diff}
	]{
		\begin{minipage}{0.3\linewidth}{\begin{center}
					\tablestyle{1.5pt}{1.2}
					\begin{tabular}{l|cccc}
                        % \shline
                        Iter & 20 & 40 & 50 \\ [.1em]
                        \shline
					FID & 16.9 & 15.7 & 15.1\\
                        % \hline
                    \end{tabular}
		\end{center}}\end{minipage}
	}
	 \subfloat[
	\textbf{Occlusion type}.
	\label{tab:occ type}
	]{
		\centering
		\begin{minipage}{0.3\linewidth}{\begin{center}
    \tablestyle{1.5pt}{1.2}
    \begin{tabular}{l|ccc}
        % \shline
        Occ. & Rectangle & Oval & Object \\ [.1em]
        \shline
    FID & 15.3 & 15.1 & 16.9 \\
        % \hline
    \end{tabular}
		\end{center}}\end{minipage}
	}
 \subfloat[
	\textbf{Availablility of complete object}.
	\label{tab:complete data}
	]{
		\centering
		\begin{minipage}{0.3\linewidth}{\begin{center}
    \tablestyle{1.5pt}{1.2}
    \begin{tabular}{l|cc}
        % \shline
        Comp. & \Checkmark & \XSolidBrush \\[.1em]
        \shline
    FID & 16.9 & 19.4 \\
        % \hline
    \end{tabular}
		\end{center}}\end{minipage}
	}\\
 \vspace{0.5cm}
 \subfloat[
	\textbf{Voting strategies}.
	\label{tab:voting}
	]{
		\begin{minipage}{0.45\linewidth}{\begin{center}
					\tablestyle{1.5pt}{1.2}
					\begin{tabular}{l|cccc}
                        % \shline
                        Strategy & Logits (V) & Logits (M)  & Mask (V)  & Mask (M)\\ [.1em]
                        \shline
					FID & 16.9 & 17.2 & 17.6 & 17.0\\
                        % \hline
                    \end{tabular}
		\end{center}}\end{minipage}
	}
  \subfloat[
	\textbf{Mask loss}.
	\label{tab:mask loss}
	]{
		\begin{minipage}{0.3\linewidth}{\begin{center}
					\tablestyle{1.5pt}{1.2}
					\begin{tabular}{l|cccc}
                        % \shline
                        $\mathcal{L}_{mask}$ & \Checkmark & \XSolidBrush \\ [.1em]
                        \shline
					FID & 16.9 & 17.7 \\
                        % \hline
                    \end{tabular}
		\end{center}}\end{minipage}
	}
	\caption{\textbf{More ablation of MaskComp.} We report the performance with the AHP dataset. (a) We ablate the iteration number of the diffusion model. (b) We report the performance with different types of occlusion. (c) We report the performance of MaskComp trained with or without the complete objects. (d) We ablate voting strategies. V: voting. M: Mean. (e) We ablate the effectiveness of adding intermediate supervision to predict the complete mask.}
 % (c) We report the performance of MaskComp trained with or without the complete objects.}
	\label{tab:more ablation}
\end{table*}}
